WakeLoc: An Ultra-Low Power, Accurate and Scalable On-Demand RTLS using Wake-Up Radios

For future large scale robotic moon missions, the availability of infrastructure-less, cheap and low power real-time locating systems (RTLSs) is critical. Traditional RTLS face significant trade-offs between power consumption and localization latency, often requiring anchors to be connected to the power grid or sacrificing speed for energy efficiency. This paper proposes WakeLoc, an on-demand RTLS based on ultra-wideband (UWB), enabling both low-latency and ultra-low power consumption by leveraging UWB wake-up radios (WuRs). In WakeLoc, tags independently start a localization procedure by sending a wake-up call (WuC) to anchors, before performing the actual localization. Distributed tags equipped with WuRs listen to the WuC and use passive listening of the UWB messages to determine their own position. Experimental measurements demonstrate that the localization accuracy in a 2D setup achieves less than 12.9cm error, both for the active and the passive tag. Additional power simulations based on real-world measurements were performed in a realistic environment, showing that anchors can achieve a power consumption as low as 15.53{\mu}W while the RTLS performs one on-demand localization per minute for 5 tags, thus operate up to 5.01 years on a single coin cell battery (690mWh).

==> content/03_background.tex <==
\section{Background}\label{sec:background}
The principles of the two protocols used as base-line are shortly explained in this section.

\begin{figure*}[htpb!]
\begin{center}
    \stackinset{l}{-2pt}{b}{-2pt}{(a)}{    \includesvg[width=0.35\textwidth]{figures/system_architecture1_converted.svg}}
    \hspace{0.1\textwidth}
    \stackinset{l}{-2pt}{b}{-2pt}{(b)}{
    \includesvg[width=0.35\textwidth]{figures/system_architecture2_converted.svg}}
    \caption{Localization based on (a) \ac{AP-TWR} (only \textit{active} part) and (b) \textsc{FlexTDOA}. Blue boxes mark transmitted messages, orange boxes mark received messages.}\label{fig:old-schemes}
\end{center}
\vspace{-5mm}
\end{figure*}

%% System architecture
\subsection[AP-TWR]{\Acl{AP-TWR}}\label{subsec:act-pass-rtls}
The \ac{AP-TWR} procedure by Laadung et al.~\cite{laadung22_novel_activ_passiv_two_way} consists of two parts: an \textit{active} localization, performed by the tag initializing the procedure and a \textit{passive} localization performed by one anchor.

The \textit{active} localization is a form of nested \ac{CC-SS-TWR}: In comparison to naive \ac{TWR}, the \ac{AP-TWR} reduces the distance measurement message exchange from at least \(N\) poll and \(N\) response messages down to \(N+1\) messages for a localization with \(N\) anchors: all the anchors respond almost simultaneously to the same poll message, as shown in~\cref{fig:old-schemes}(a). This means that only \(N+1\) messages need to be exchanged in total.

The \textit{passive} localization is not further considered in our work, as it comes with a significant overhead of the final message sent by the tag.

This scheme allows scalability in the number of anchors and privacy protection. It scales both, in number of anchors and setup complexity. The anchors only need to know their own position, but never communicate with each other. If a new anchor is added, neither provisioning nor an adjustment of the communication structure is required - the new anchor can immediately work as an anchor, provided its position is known. 

On the tag side the \ac{AP-TWR} allows for an energy efficient implementation: Since they localize themselves independently of a global schedule, it is sufficient for them to wake up briefly, send their poll message and wait for at least four anchor responses. Tags can start localization on their own, guaranteeing therefore on-demand capabilities by maintaining their own privacy as the calculations are carried out exclusively on the tags.

However, on the anchor side, this scheme can not be implemented efficiently, as the anchor's receiver has to be always-on in order to provide the on-demand functionality to the tag. Additionally, with many tags actively polling for measurements, collisions occur and thus scalability in the number of tags is not given.

\subsection{DL-TDOA and FlexTDOA}\label{subsec:flextdoa}
In contrast to \ac{AP-TWR}, \ac{DL-TDOA}~\cite{santoro21_scale} requires the anchors \(A_i\) to be time-synchronized and sending time-synchronized messages. The tag \(T\) measures the arrival time of these anchor messages, calculates its distance to the anchors by \acl{TDOA}, and thus localizes itself. The distances between the tag and the anchors are described by~\cref{eq:tdoa}, where \(\mathrm{c}\) is the speed of light, \(t_{TA_iA_j}\) the \acl{TDOA} between the tag \(T\), anchor \(A_i\) and anchor \(A_j\), and \(d_{TA_i}\) the distance between tag \(T\) and anchor \(A_i\).
\begin{equation}\label{eq:tdoa}
  t_{TA_iA_j}=\frac{d_{TA_i}-d_{TA_j}}{\mathrm{c}}
\end{equation}
If the position of the anchors are known and at least 4 \ac{TDOA} measurements are available, the 3D location of the tag can be calculated. The tags can thereby be completely \textit{passive} receivers, with no difference to the amount of tags localizing themselves. However, the anchors need to be very well synchronized (a \qty{1}{\nano\second} delay results in a distance error of \(\approx\qty{30}{\centi\meter}\)). Furthermore, tags are dependent on the localization period of the \ac{RTLS}.

Classically, the time synchronization between the anchors is performed by choosing one anchor as reference and consequently trimming the transceiver crystal skew of all other anchors to match the same frequency. This is energy-intensive for the anchors, since they have to
\begin{enumerate*}[label=\textit{\roman*)}]
\item constantly receive synchronization packets to correct drifts and
\item keep the transceivers' \ac{PLL} running to maintain time synchronization.
\end{enumerate*}
Especially for larger deployments the time synchronization has to be forwarded to anchors outside of the \ac{UWB} range of the reference anchor, creating high coordination complexity in such deployments.


% FlexTdoa
To mitigate these issues, an energy-efficient approach to \ac{DL-TDOA} is presented by Patru et al.~\cite{patru23_flext} with \textsc{FlexTDOA}: By exploiting the \ac{CFO} error correction, they implemented a synchronization-free \ac{DL-TDOA} without compromising accuracy. An initiator anchor \(A_0\) sends a first message, and starts the \ac{TDOA} procedure. The following anchors \(A_1\) to \(A_N\) receive this poll message, and send a response message themselve after a wait period \(\Delta T_i\), as shown in~\cref{fig:old-schemes}(b).

A tag that wants to localize itself can now listen to all these measurements and calculate its own position using \ac{TDOA}, the known \(\Delta T_i\), positions \(\vec{X}_i\) as well as the \ac{CFO} of each anchor with respect to the tag. Using a static particle filter as described in~\cite{gustafsson03_positioning_tdoa}, the non-linear least squares problem can be solved very efficiently on a microcontroller.

This scheme can be implemented very power efficiently for both the anchors and tags: Using a global localization schedule, the anchors and tags wake-up periodically (period \(T_F\)) and perform a \ac{TDOA} procedure. Additionally, the scheme is easily scalable in the number of tags, as they are completely \textit{passive} and thus no message collisions can happen. However,
\begin{enumerate*}[label=\textit{\roman*)}]
  \item for large-scale setups a lot of coordination between the anchors is needed to choose the initiator, and new anchors need a provisioning to be part of the anchors;
  \item a trade-off between localization latency and power consumption has to be made. In particular, anchors cannot determine the desired localization frequency of the tags; and
  \item there is no spatial awareness of the anchors as to whether tags are in the vicinity and whether localization is required at all, thus discarding energy saving options.
\end{enumerate*}

